Enhancing Federated Learning Convergence with Dynamic Data Queue and Data Entropy-driven Participant Selection

Federated Learning (FL) is a decentralized approach for collaborative model training on edge devices. This distributed method of model training offers advantages in privacy, security, regulatory compliance, and cost-efficiency. Our emphasis in this research lies in addressing statistical complexity in FL, especially when the data stored locally across devices is not identically and independently distributed (non-IID). We have observed an accuracy reduction of up to approximately 10\% to 30\%, particularly in skewed scenarios where each edge device trains with only 1 class of data. This reduction is attributed to weight divergence, quantified using the Euclidean distance between device-level class distributions and the population distribution, resulting in a bias term (\(\delta_k\)). As a solution, we present a method to improve convergence in FL by creating a global subset of data on the server and dynamically distributing it across devices using a Dynamic Data queue-driven Federated Learning (DDFL). Next, we leverage Data Entropy metrics to observe the process during each training round and enable reasonable device selection for aggregation. Furthermore, we provide a convergence analysis of our proposed DDFL to justify their viability in practical FL scenarios, aiming for better device selection, a non-sub-optimal global model, and faster convergence. We observe that our approach results in a substantial accuracy boost of approximately 5\% for the MNIST dataset, around 18\% for CIFAR-10, and 20\% for CIFAR-100 with a 10\% global subset of data, outperforming the state-of-the-art (SOTA) aggregation algorithms.

==> references.tex <==
\bibitem{FLOpt2015}
Jakub Kone{\v{c}}n{\'y}, B McMahan, Daniel Ramage.
"Federated Optimization: Distributed Optimization Beyond the Datacenter."
\textit{CoRR}, vol. abs/1511.03575, 2015.
Available: \url{http://arxiv.org/abs/1511.03575}

\bibitem{ComEff2017}
H. Brendan McMahan, Eider Moore, Daniel Ramage, Blaise Ag{\"{u}}era y Arcas.
"Federated Learning of Deep Networks using Model Averaging."
\textit{CoRR}, vol. abs/1602.05629, 2016.
Available: \url{http://arxiv.org/abs/1602.05629}

\bibitem{FLMulti2017}
Virginia Smith, Chao{-}Kai Chiang, Maziar Sanjabi, Ameet Talwalkar.
"Federated Multi-Task Learning."
\textit{CoRR}, vol. abs/1705.10467, 2017.
Available: \url{http://arxiv.org/abs/1705.10467}

\bibitem{FLhealth2019}
Zhiang Xu, Yijia Guo, Chinmay Chakraborty, Qiaozhi Hua, Shengbo Chen, Keping Yu.
"A Simple Federated Learning-Based Scheme for Security Enhancement Over Internet of Medical Things."
\textit{IEEE Journal of Biomedical and Health Informatics}, vol. 27, no. 2, pp. 652-663, 2023.
doi: 10.1109/JBHI.2022.3187471.

\bibitem{FLforMbKey2018}
Andrew Hard, Kanishka Rao, Rajiv Mathews, Fran{\c{c}}oise Beaufays, Sean Augenstein, Hubert Eichner, Chlo{\'{e}} Kiddon, Daniel Ramage.
"Federated Learning for Mobile Keyboard Prediction."
\textit{CoRR}, vol. abs/1811.03604, 2018.
Available: \url{http://arxiv.org/abs/1811.03604}

\bibitem{Junchuan2022}
Lingjuan Lyu, Han Yu, Xingjun Ma, Chen Chen, Lichao Sun, Jun Zhao, Qiang Yang, Philip S. Yu.
"Privacy and Robustness in Federated Learning: Attacks and Defenses."
\textit{IEEE Transactions on Neural Networks and Learning Systems}, 2022.
doi: 10.1109/TNNLS.2022.3216981.

\bibitem{niidconvergence2020}
Xiang Li, Kaixuan Huang, Wenhao Yang, Shusen Wang, Zhihua Zhang.
"On the Convergence of FedAvg on Non-IID Data."
\textit{8th International Conference on Learning Representations (ICLR)}, 2020.
Available: \url{https://openreview.net/forum?id=HJxNAnVtDS}

\bibitem{FLnIIDDataSilos2022}
Qinbin Li, Yiqun Diao, Quan Chen, Bingsheng He.
"Federated Learning on Non-IID Data Silos: An Experimental Study."
\textit{CoRR}, vol. abs/2102.02079, 2021.
Available: \url{https://arxiv.org/abs/2102.02079}

\bibitem{FLEdgeInt2023}
Aristeidis Karras, Christos Karras, Konstantinos C. Giotopoulos, Dimitrios Tsolis, Konstantinos Oikonomou, Spyros Sioutas.
"Federated Edge Intelligence and Edge Caching Mechanisms."
\textit{Information}, vol. 14, no. 7, article 414, 2023.
doi: 10.3390/info14070414.

\bibitem{FLOptNiid2020}
Hao Wang, Zakhary Kaplan, Di Niu, Baochun Li.
"Optimizing Federated Learning on Non-IID Data with Reinforcement Learning."
\textit{IEEE INFOCOM 2020 - IEEE Conference on Computer Communications}, 2020, pp. 1698-1707.
doi: 10.1109/INFOCOM41043.2020.9155494.

\bibitem{FLComEff2016}
Jakub Kone{\v{c}}n{\'y}, H. Brendan McMahan, Felix X. Yu, Peter Richt{\'{a}}rik, Ananda Theertha Suresh, Dave Bacon.
"Federated Learning: Strategies for Improving Communication Efficiency."
\textit{CoRR}, vol. abs/1610.05492, 2016.
Available: \url{http://arxiv.org/abs/1610.05492}

\bibitem{FlNiid2018}
Yue Zhao, Meng Li, Liangzhen Lai, Naveen Suda, Damon Civin, Vikas Chandra.
"Federated Learning with Non-IID Data."
\textit{CoRR}, vol. abs/1806.00582, 2018.
Available: \url{http://arxiv.org/abs/1806.00582}

\bibitem{FedMD2019}
Daliang Li, Junpu Wang.
"FedMD: Heterogenous Federated Learning via Model Distillation."
\textit{CoRR}, vol. abs/1910.03581, 2019.
Available: \url{http://arxiv.org/abs/1910.03581}

\bibitem{icc_conf_client_selection}
Takayuki Nishio and Ryo Yonetani.
"Client Selection for Federated Learning with Heterogeneous Resources in Mobile Edge."
\textit{CoRR}, vol. abs/1804.08333, 2018.
Available: \url{http://arxiv.org/abs/1804.08333}

\bibitem{warmup2022}
Mohamad Wazzeh, Hakima Ould-Slimane, Chamseddine Talhi, Azzam Mourad, and Mohsen Guizani.
"Warmup and Transfer Knowledge-Based Federated Learning Approach for IoT Continuous Authentication."
\textit{CoRR}, 2022.
Available: \url{http://arxiv.org/abs/2211.05662}

\bibitem{FedAvg2017}
H. Brendan McMahan, Eider Moore, Daniel Ramage, and Blaise Ag{\"{u}}era y Arcas.
"Federated Learning of Deep Networks using Model Averaging."
\textit{CoRR}, vol. abs/1602.05629, 2016.
Available: \url{http://arxiv.org/abs/1602.05629}

\bibitem{defKt2022}
Chengxi Li, Gang Li, and Pramod K. Varshney.
"Decentralized Federated Learning via Mutual Knowledge Transfer."
\textit{IEEE Internet of Things Journal}, vol. 9, no. 2, pp. 1136-1147, 2022.
doi: 10.1109/JIOT.2021.3078543.

\bibitem{FLConApps2019}
Qiang Yang, Yang Liu, Tianjian Chen, and Yongxin Tong.
"Federated Machine Learning: Concept and Applications."
\textit{CoRR}, vol. abs/1902.04885, 2019.
Available: \url{http://arxiv.org/abs/1902.04885}

\bibitem{OnConvFL2018}
Anit Kumar Sahu, Tian Li, Maziar Sanjabi, Manzil Zaheer, Ameet Talwalkar, and Virginia Smith.
"On the Convergence of Federated Optimization in Heterogeneous Networks."
\textit{CoRR}, vol. abs/1812.06127, 2018.
Available: \url{http://arxiv.org/abs/1812.06127}

\bibitem{OpenProbFL2019}
Peter Kairouz, H. Brendan McMahan, Brendan Avent, et al.
"Advances and Open Problems in Federated Learning."
\textit{CoRR}, vol. abs/1912.04977, 2019.
Available: \url{http://arxiv.org/abs/1912.04977}

\bibitem{Reza2016}
Reza Shokri and Vitaly Shmatikov.
"Privacy-preserving Deep Learning."
In \textit{53rd Annual Allerton Conference on Communication, Control, and Computing (Allerton)}, pp. 909-910, 2015.
doi: 10.1109/ALLERTON.2015.7447103.

\bibitem{FLEdge2022}
Haftay Gebreslasie Abreha, Mohammad Hayajneh, and Mohamed Adel Serhani.
"Federated Learning in Edge Computing: A Systematic Survey."
\textit{Sensors}, vol. 22, no. 2, article 450, 2022.
doi: 10.3390/s22020450.

\bibitem{fairness_guarantee}
Tiansheng Huang, Weiwei Lin, Wentai Wu, Ligang He, Keqin Li, and Albert Y. Zomaya.
"An Efficiency-boosting Client Selection Scheme for Federated Learning with Fairness Guarantee."
\textit{CoRR}, vol. abs/2011.01783, 2020.
Available: \url{https://arxiv.org/abs/2011.01783}

\bibitem{euc2023}
Charuka Herath, Yogachandran Rahulamathavan, and Xiaolan Liu.
"Recursive Euclidean Distance-based Robust Aggregation Technique for Federated Learning."
In \textit{IEEE IAS Global Conference on Emerging Technologies (GlobConET)}, 2023, pp. 1-6.
doi: 10.1109/GlobConET56651.2023.10150168.

\bibitem{FairFL2019}
Tian Li, Maziar Sanjabi, and Virginia Smith.
"Fair Resource Allocation in Federated Learning."
\textit{CoRR}, vol. abs/1905.10497, 2019.
Available: \url{http://arxiv.org/abs/1905.10497}

\bibitem{infoEntopy2013}
Jianbo Gao, Feiyan Liu, Jianfang Zhang, Jing Hu, and Yinhe Cao.
"Information Entropy As a Basic Building Block of Complexity Theory."
\textit{Entropy}, vol. 15, no. 9, pp. 3396--3418, 2013.
doi: 10.3390/e15093396.

\bibitem{PPTraficIoT2020}
Liu, Y., Yu, J. J. Q., Kang, J., Niyato, D., and Zhang, S.
"Privacy-Preserving Traffic Flow Prediction: A Federated Learning Approach". 
\textit{IEEE Internet of Things Journal}, 7(8), 7751-7763, 2020.
doi:10.1109/JIOT.2020.2991401.

\bibitem{ComEffIoT2020}
Mills, J., Hu, J., and Min, G. (2020). Communication-Efficient Federated Learning for Wireless Edge Intelligence in IoT. \textit{IEEE Internet of Things Journal}, 7(7), 5986-5994. doi:10.1109/JIOT.2019.2956615.

\bibitem{CIFAR-10}
Krizhevsky, A., and  Hinton, G. (2009). Learning multiple layers of features from tiny images. \textit{Technical report, University of Toronto, Toronto, Ontario}. Retrieved from https://www.cs.toronto.edu/~kriz/learning-features-2009-TR.pdf.

\bibitem{MNIST}
Lecun, Y., Bottou, L., Bengio, Y., and  Haffner, P. (1998). Gradient-based learning applied to document recognition. \textit{Proceedings of the IEEE}, 86(11), 2278-2324. doi:10.1109/5.726791.

\bibitem{du2022gradient}
Du, J., Jiang, B., Jiang, C., Shi, Y., and  Han, Z. (2022). Gradient and Channel Aware Dynamic Scheduling for Over-the-Air Computation in Federated Edge Learning Systems. arXiv preprint arXiv:2212.00491.

\bibitem{minJoingLer2019}
Chen, M., Yang, Z., Saad, W., Yin, C., Poor, H. V., and  Cui, S. (2019). A Joint Learning and Communications Framework for Federated Learning over Wireless Networks. \textit{CoRR}, abs/1909.07972. Retrieved from http://arxiv.org/abs/1909.07972.

\bibitem{FLChallenges2020}
Li, T., Sahu, A. K., Talwalkar, A., and  Smith, V. (2020). Federated Learning: Challenges, Methods, and Future Directions. \textit{IEEE Signal Processing Magazine}, 37(3), 50-60. doi:10.1109/MSP.2020.2975749.

\bibitem{FedML2020}
He, C., Li, S., So, J., Zhang, M., Wang, H., Wang, X., Vepakomma, P., Singh, A., Qiu, H., Shen, L., Zhao, P., Kang, Y., Liu, Y., Raskar, R., Yang, Q., Annavaram, M., and  Avestimehr, S. (2020). FedML: A Research Library and Benchmark for Federated Machine Learning. \textit{CoRR}, abs/2007.13518. Retrieved from https://arxiv.org/abs/2007.13518.

\bibitem{AccurateDib2018}
Maniruzzaman, M., Rahman, M. J., Hasan, A. M., et al. (2018). Accurate Diabetes Risk Stratification Using Machine Learning: Role of Missing Value and Outliers. \textit{Journal of Medical Systems}, 42. doi: https://doi.org/10.1007/s10916-018-0940-7.

\bibitem{LiuBatchSize2020}
Liu, S., Yu, G., Yin, R., Yuan, J., and  Qu, F. (2020). Adaptive Batchsize Selection and Gradient Compression for Wireless Federated Learning. In \textit{GLOBECOM 2020 - 2020 IEEE Global Communications Conference} (pp. 1-6). doi:10.1109/GLOBECOM42002.2020.9322122.

\bibitem{batchsize2022}
Zhang, J., Guo, S., Qu, Z., Zeng, D., Zhan, Y., Liu, Q., and  Akerkar, R. (2022). Adaptive Federated Learning on Non-IID Data With Resource Constraint. \textit{IEEE Transactions on Computers}, 71(7), 1655-1667. doi:10.1109/TC.2021.3099723.

\bibitem{comeff_2013}
Zhang, Y., Duchi, J. C., and  Wainwright, M. J. (2013). Communication-efficient algorithms for statistical optimization. \textit{Journal of Machine Learning Research}, 14(1), 3321-3363.

\bibitem{stich_2018}
Lin, T., Stich, S. U., and  Jaggi, M. (2018). Don't Use Large Mini-Batches, Use Local SGD. \textit{CoRR}, abs/1808.07217. Retrieved from http://arxiv.org/abs/1808.07217.

\bibitem{Sahu_2018}
Sahu, A. K., Li, T., Sanjabi, M., Zaheer, M., Talwalkar, A., and  Smith, V. (2018). On the Convergence of Federated Optimization in Heterogeneous Networks. \textit{CoRR}, abs/1812.06127. Retrieved from http://arxiv.org/abs/1812.06127.

\bibitem{Li_2019}
Li, X., Huang, K., Yang, W., Wang, S., and  Zhang, Z. (2020). On the Convergence of FedAvg on Non-IID Data. In \textit{International Conference on Learning Representations}. Retrieved from https://openreview.net/forum?id=HJxNAnVtDS.



